Coffee-Gym: An Environment for Evaluating and Improving Natural Language Feedback on Erroneous Code

This paper presents Coffee-Gym, a comprehensive RL environment for training models that provide feedback on code editing. Coffee-Gym includes two major components: (1) Coffee, a dataset containing humans' code edit traces for coding questions and machine-written feedback for editing erroneous code; (2) CoffeeEval, a reward function that faithfully reflects the helpfulness of feedback by assessing the performance of the revised code in unit tests. With them, Coffee-Gym addresses the unavailability of high-quality datasets for training feedback models with RL, and provides more accurate rewards than the SOTA reward model (i.e., GPT-4). By applying Coffee-Gym, we elicit feedback models that outperform baselines in enhancing open-source code LLMs' code editing, making them comparable with closed-source LLMs. We make the dataset and the model checkpoint publicly available.

==> figure_latex/coffee_gym_validate_HE.tex <==
\begin{figure}[!ht]
\centering
    \includegraphics[width=1.0\linewidth]{figures/CGV-HE.pdf}

\caption{End-to-end validation results of reference methods in \coffeegym. We report the Pass@1 score of \textsc{Coffee-Test}.}
\label{fig:coffeegym_validate_HE}
\end{figure}

==> figure_latex/coffee_pass_ratio.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/pass-ratio.pdf}    
    \caption{Pass@1 result of SFT critic $\theta$ on the test set of \textsc{Coffee}. The performance has decreased even when it is compared with No Feedback setting and there is a significant gap between ChatGPT Feedback and SFT Feedback.}
\label{fig:pass_ratio}
\end{figure}

==> figure_latex/figure_critic_amt.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=0.92\linewidth]{figures/humaneval_critic_inferface_amt.png}
\caption{The interface used for human evaluation on the quality of feedback generated from critic.} 
\label{fig:amt_prelim}
\end{figure*}


==> figure_latex/training_method_analysis.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=1.0\linewidth]{figures/training_method_analysis.pdf}
\caption{Reference methods analysis results on HumanEvalFix (Pass@1). The DeepSeek-Coder-7b~\citep{Guo2024DeepSeekCoderWT} model is utilized as the code editor.} 
\label{fig:training_method_analysis}
\end{figure}

